Open-PMC-18M: A High-Fidelity Large Scale Medical Dataset for Multimodal Representation Learning

In biomedical vision-language modeling, datasets are typically mined from scientific literature, pairing compound figures with captions that are short, context-dependent, and oftern partially informative. Prior work on subfigure extraction has been limited in both dataset size and generalizability. In addition, no existing effort has incorporated rich medical context in image-text pairs. We revisit data curation as a foundational component of effective biomedical representation learning. Our data curation process integrates transformer-based subfigure detection, subcaption extraction, and contextual text enrichment derived from inline references. Our subfigure extraction model, trained on a corpus of 500,000 compound figures, achieves state-of-the-art performance on real and synthetic benchmarks. Using this process, we curate and release Open-PMC-18M, a large-scale high-fidelity biomedical dataset comprising 18 million image-text pairs, spanning radiology, microscopy, and visible light photography. We train vision-language models on our dataset and perform extensive evaluation on 6 retrieval and 19 zero-shot classification tasks across three major modalities. The models trained on our dataset set a new state-of-the-art results in medical representation learning. We release our dataset, models, and code to support reproducible benchmarks and further study into biomedical vision-language modeling and representation learning.

==> CVPR/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> CVPR/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> CVPR/sec/0_abstract.tex <==
\begin{abstract}
Compound figures, which are multi-panel composites containing diverse subfigures, are ubiquitous in biomedical literature, yet large-scale subfigure extraction remains largely unaddressed. Prior work on subfigure extraction has been limited in both dataset size and generalizability, leaving a critical open question: \textit{How does high-fidelity image–text alignment via large-scale subfigure extraction impact representation learning in vision-language models?} We address this gap by introducing a scalable subfigure extraction pipeline based on transformer-based object detection, trained on a synthetic corpus of 500,000 compound figures, and achieving state-of-the-art performance on both ImageCLEF 2016 and synthetic benchmarks. Using this pipeline, we release \textbf{\datasetsub}, a large-scale high quality biomedical vision-language dataset comprising \textit{18 million} clinically relevant subfigure–caption pairs spanning radiology, microscopy, and visible light photography. We train and evaluate vision-language models on our curated datasets and show improved performance across retrieval, zero-shot classification, and robustness benchmarks, outperforming existing baselines. We release our dataset, models, and code to support reproducible benchmarks and further study into biomedical vision-language modeling and representation learning.
\end{abstract}

==> CVPR/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

The rapid progress of general-domain vision-language models (VLM) \citep{radford2021learning,jia2021scaling,girdhar2023imagebind} has sparked growing interest in building large-scale multimodal datasets tailored to the medical domain \citep{zhang2023biomedclip,lin2023pmc,pelka2018radiology,lozano2025biomedica,openpmc}. Despite these efforts, the scale of medical datasets still lags far behind their general-domain counterparts. While increasing dataset \textit{size} continues to be a primary goal, there is growing recognition that improving the \textit{quality} and \textit{relevance} of image-text pairs may be a more effective strategy for enhancing model performance and clinical utility \citep{openpmc}.

Biomedical figures present unique challenges: they often consist of compound layouts that combine multiple subfigures, each potentially depicting a different imaging modality, anatomical region, or clinical concept. Unlike dataset scale, which has received substantial attention, this structural heterogeneity remains largely unexplored. Most of the existing biomedical VLM pipelines treat compound figures as atomic units, pairing the entire image with a caption, without disentangling their internal structure.

We hypothesize that such coarse image-text alignment could introduce noise into pretraining, ultimately impacting the transferability and generalizability of the learned representations. While recent work has scaled data curation through bulk mining of PubMed Central (PMC)\footnote{https://pmc.ncbi.nlm.nih.gov/} articles (e.g., \biomedclip \citep{zhang2023biomedclip} and \biomedica \citep{lozano2025biomedica}), these efforts still rely on noisy and compound figures. To our knowledge, only a few prior works incorporate subfigure extraction as part of the curation process \citep{pelka2018radiology,lin2023pmc,openpmc}; however, they do so at small scale. This raises an important gap in the field: \textit{how does subfigure extraction and the resulting improvement in medical image-text alignment quality impact representation learning at scale, particularly given the known sensitivity of contrastive objectives to both dataset size and alignment fidelity during pretraining?}

In this work, we investigate the impact of large-scale subfigure extraction on medical vision-language representation learning. We first create a dataset of 6 million image-caption pairs by filtering out non-medical images (e.g., charts, plots, tables) from the BIOMEDICA corpus \citep{lozano2025biomedica} using a combination of label metadata and a ResNet classifier. For the \textit{subfigure extraction} step, we train a high-performance object detection model with the same architecture as DAB-DETR (Dynamic Anchor Boxes DEtection TRansformer) \citep{liu2022dabdetr} on a corpus of 500,000 programmatically-created compound figures. By decomposing compound figures with this model, we build \datasetsub, one of the largest and most curated collections of biomedical image-text pairs to date, consisting of 18 million subfigure-caption pairs. We then train vision and text encoders using a contrastive learning objective and evaluate the resulting models on an extensive suite of downstream tasks, including cross-modal retrieval and zero-shot classification across three distinct medical modalities: radiology, microscopy, and visible light photography (VLP). We release our dataset\footnote{https://huggingface.co/datasets/vector-institute/open-pmc-18m}, models, and code\footnote{https://anonymous.4open.science/r/open-pmc-18m-CE25/} to support reproducible benchmarks and further study into biomedical VLM and representation learning. Our contributions are as follows:
\begin{itemize}
    \item We propose a scalable subfigure extraction pipeline using transformer-based object detection trained on a 500,000 compound figure dataset, achieving state-of-the-art performance on ImageCLEF 2016 \citep{KGD2014,GSB2016} and synthetic evaluation sets.
    \item We release \datasetsub, a large-scale biomedical image-text dataset with 18 million subfigure-caption pairs filtered for clinical relevance across radiology, microscopy, and visible light photography.
    \item We provide a comprehensive evaluation of vision-language models trained on our datasets, demonstrating improved performance in retrieval, classification, and robustness across multiple medical benchmarks.
\end{itemize}



==> CVPR/sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Biomedical Vision-Language Datasets}
Most efforts to date have relied on mining figures and captions from the PMC Open Access subset.\footnote{https://pmc.ncbi.nlm.nih.gov/tools/openftlist/} One of the earliest publicly available datasets is ROCO \citep{pelka2018radiology}, which compiled around 80,000 radiology and 6,000 non-radiology images, enriched with metadata such as captions and keywords. Later, \citet{lin2023pmc} introduced PMC-OA , which includes 1.6 million image-text pairs. Their contribution emphasized automation—proposing a pipeline to streamline the pairing process and reduce human annotation. More recently, \citet{zhang2023biomedclip} announced \biomedclip, a dataset of 15 million image-text pairs. The largest released dataset to date is \biomedica \citep{lozano2025biomedica}, which comprises 24 million pairs and employs clustering, vision encoders, and expert taxonomies to assign modality labels at global and local levels. While these efforts represent major progress in scale, recent work has emphasized that data quality is a critical factor in learning effective and generalizable medical representations \citep{openpmc}. Building on the premise of \datasetsmall, our work takes a quality-first approach while also significantly scaling up the dataset. %\arash{The rest of this paragraph should be moved out of Related work.}We expand the corpus nearly nine-fold, constructing a high-quality biomedical image-text dataset with broader coverage across imaging modalities and clinical subdomains. In parallel, we improve subfigure segmentation by training a multimodal panel detector that extends prior work with enhanced support for microscopy images—a modality underrepresented or misclassified in earlier segmentation efforts. This detector is trained on a large synthetic corpus and applied to compound figures across PMC, enabling robust and scalable subfigure-level pairing that preserves both visual and semantic granularity.

\subsection{Subfigure Extraction as Object Detection}
Early approaches to compound figure separation relied on classical computer vision techniques, using heuristics based on whitespace, edge detection, or layout regularity. However, these methods often struggled to handle diverse panel styles and complex spatial arrangements. More recent work treats subfigure extraction as an object detection problem, leveraging deep learning models. For example, \citet{tsutsui2017data} and \citet{yao2021compound} used YOLO for subfigure separation. \citet{lin2023pmc} also uses an object detection model to extract subfigures in their pipeline. They train a DETR (DEtection TRansformer) \citep{carion2020end} model on the MedICaT dataset \citep{subramanian2020medicat} containing 2069 annotated compound figures.

Data annotation for training an image decomposition model is challenging and time-consuming. Current annotated datasets for this are small, which lead to models with suboptimal performance. To overcome this, synthetic datasets of compound figures have been proposed, where subfigures are programmatically composed to simulate real-world layouts. This allows training of object detection models without relying on large-scale human-annotated data \citep{tsutsui2017data, yao2021compound}. %\arash{The rest of the paragraph should be moved out of Related Work} Our work builds on this line of research by generating a large-scale synthetic dataset of 500K compound figures for training a high-performance DAB-DETR model. We demonstrate that this detector generalizes well to real PMC figures and enables scalable subfigure decomposition, yielding over 18M image-caption pairs.



==> CVPR/sec/3_data.tex <==
\section{Data Composition and Curation Process}
\label{sec:data}
\subsection{Initial Collection and Filtering}

We begin with the \biomedica dataset \citep{lozano2025biomedica}, which has been extracted from articles in the PubMed Central Open Access Subset. \biomedica contains approximately 24 million image-caption pairs along with metadata, including global and local modality labels for each image. We apply a filtering step using the provided labels and retain only those pairs primarily categorized as clinical imaging, microscopy, immunoassays, or chemical structure. This yields a dataset of 6 million pairs, which we refer to as \datasetcomp in this paper.

\subsection{Vision-Based Subfigure Extraction} \label{detr}
To enable scalable extraction of subfigures from biomedical compound figures, we trained a transformer-based object detection architecture, Dynamic Anchor Box DEtection TRansformer (DAB-DETR) \citep{liu2022dabdetr}. Prior work of \citet{lin2023pmc} trained a DETR model on MedICaT \citep{subramanian2020medicat} with only 2,069 manually annotated compound figures. In contrast, we trained our model on a large-scale synthetic dataset of 500,000 compound figures, the first of its kind in the biomedical domain. We use DAB-DETR as it improves upon the original DETR model by learning dynamic anchors as queries, resulting in improved localization and faster convergence \citep{liu2022dabdetr}.


%To enable automated extraction of individual subfigures from compound figures, we developed an object detection model based on the DEtection TRansformer (DETR) architecture. The objective was to locate and segment subfigures within larger, composite images typically found in scientific literature. Our approach reframes subfigure detection as a direct set prediction problem, where the model simultaneously predicts the number, location, and bounding boxes of subfigures without relying on hand-crafted proposals or post-processing steps.
\paragraph{Synthetic Data Formation.} To train a subfigure extraction model at scale, we generate a synthetic dataset by reversing the subfigure extraction process: rather than decomposing existing compound figures, we programmatically construct new ones by composing multiple single-panel biomedical images into compound layouts. The key advantage of this approach is the availability of ground-truth bounding boxes for each subfigure. Our generation pipeline samples a layout template that specifies the spatial arrangement of subfigures. Each layout is defined by a set of configurable parameters, including:
% (Figure \ref{fig:layout}):
\begin{itemize}
\setlength\itemsep{0.1em}
\item \textbf{Grid Size}: Specifies a standard $m \times n$ grid or a custom arrangement for panel placement.
\item \textbf{Margins}: Random horizontal and vertical spacing between panels to simulate variability in published figure layouts.
\item \textbf{Labeling Scheme}: Determines how panels are annotated (e.g., using numerical, alphabetical, or compound labels like "1a" or "a-1"), and whether labels appear inside or outside panel boundaries.
\item \textbf{Aspect Ratio}: Specifies a fixed width-to-height ratio applied uniformly to all subfigures.
\end{itemize}

Subfigures are sampled from a repository of single-panel biomedical images spanning diverse modalities such as radiology, microscopy, pathology, etc., which we will describe below. Composite figures may contain panels from the same modality or a heterogeneous mix, providing semantic diversity and mimicking real-world figure complexity. Figure \ref{fig:example}) illustrates the full synthetic data pipeline.

\begin{figure*}[tb]
\centering
\includegraphics[width=0.95\textwidth]{figure/layout.pdf}
\caption{\textbf{Left} Overview of our pipeline for creating synthetic compound figures used to train the DAB-DETR model. A 
\textit{Sampler} selects single-panel images and layout specifications from their respective pools. A \textit{Labeler} assigns subfigure labels from a predefined label pool (e.g., 1, a, a1, a-1), placing them according to the chosen scheme. \textbf{Right} Distribution of medical image modalities, number of subfigures per compound figure, and caption length statistics within \datasetsub. The average caption contains 165.82 tokens, with a max of 7352 and almost 19.48\% of captions had more than 256 tokens. }
\label{fig:layout}
\end{figure*}

\paragraph{Image Decomposition Model Training and Evaluation.}
We train a DAB-DETR model on the 500,000 synthetic compound figures and validate its performance on a similarly created holdout set of 20,000 images. Source subfigures are drawn from well-known benchmark datasets such as ROCO \citep{pelka2018radiology}, SICAP \citep{ESTEBAN2019303}, HAM10000 \citep{tschandl2018ham10000}, PathMNIST and RetinaMNIST from MedMNIST \citep{medmnistv1, medmnistv2}, PAD-UFES-20 \citep{pacheco2020pad}, and PlotQA \citep{Methani_2020_WACV} as listed in Table~\ref{tab:single_panel_datasets}. To ensure balanced representation, each modality-specific dataset contributes approximately 16.7\% of the total examples, with the remaining 16.7\% comprising mixed-modality compound figures. This configuration promotes both visual diversity and generalization across biomedical imaging types. Training is performed over $40$ epochs using a batch size of $64$ and an initial learning rate of $1e^{-5}$. \elham{We evaluate performance on both our synthetic validation set and the ImageCLEF 2016 compound figure separation benchmark \citep{KGD2014, GSB2016}}. Our model outperforms the model trained on MedICaT only on both evaluation sets as shown by Table~\ref{tab: subfigure_evaluation}. Figure~\ref{fig:example} showcases examples from the ImageCLEF 2016 dataset and from a subset of \datasetcomp, illustrating accurate detection of distinct subfigures across diverse panel layouts and content types.

\begin{figure*}[tb]
\centering
\includegraphics[width=0.99\textwidth]{figure/examples.pdf}
\caption{Qualitative results of subfigure detection using our DAB-DETR model. \textbf{Left} Real-world biomedical compound figures from PMC articles in \datasetcomp (also \biomedica). \textbf{Right} Examples from the ImageCLEF 2016 benchmark. The model accurately localizes and separates distinct subfigures, including heterogeneous panels and non-uniform layouts.}
\label{fig:example}
\end{figure*}

\iffalse
\negin{

\begin{figure}[tb]
\centering
\includegraphics[width=0.99\textwidth]{ICLR/figure/figure_decomp.pdf}
\caption{\textbf{Left} Qualitative results of subfigure detection using our DAB-DETR model. Real-world biomedical compound figures from PMC articles in \datasetcomp (also \biomedica). \textbf{Right} compound figures used to train the DAB-DETR model. A 
\textit{Sampler} selects single-panel images and layout specifications from their respective pools. A \textit{Labeler} assigns subfigure labels from a predefined label pool (e.g., 1, a, a1, a-1), placing them according to the chosen scheme.}
\label{fig:example}
\end{figure}

}



\begin{table*}[h]
    \centering
    \caption{Datasets used for synthetic subfigure generation, categorized by modality and split.}
    \renewcommand{\arraystretch}{1.2}  % Increase vertical spacing
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccc}
        \hline
        \textbf{Split} & \textbf{Radiology} & \textbf{Histopathology} & \textbf{Dermatology} & \textbf{Retina} & \textbf{Plots} \\
        \hline
        \textbf{Train} & ROCO & SICAP & HAM10000 & RetinaMNIST & PlotQA \\
        \textbf{Sample Size} & 65422 & 18783 & 10015 & 1080 & 60000 \\
        \hline
        \textbf{Validation} & ROCO (test) & PathMNIST & PAD-UFES-20 & RetinaMNIST (val) & PlotQA (val) \\
        \textbf{Sample Size} & 8176 & 10004 & 2298 & 120 & 10000 \\
        \hline
    \end{tabular}%
    }
    
    \label{tab:single_panel_datasets}
\end{table*}
\fi
\begin{table}[h]
    \centering
    \caption{Datasets used for synthetic subfigure generation, categorized by modality and split. $^{*}$ for ROCO the test; $^{+}$ the validation set}
    \setlength{\tabcolsep}{2pt} 
    \begin{tabular}{lcc}
        \hline
        \textbf{Modality} & \textbf{Train (Examples)}& \textbf{Validation (Examples)} \\
        \hline
        \textbf{Radiology} & ROCO (65422) & ROCO$^{*}$ (8176) \\
        \textbf{Histopathology} & SICAP (18783) & PathMNIST (10004 \\
        \textbf{Dermatology} & HAM10000 (10015) & PAD-UFES-20 (2298) \\
        \textbf{Retina} & RetinaMNIST (1080) & RetinaMNIST$^{+}$ (120) \\
        \textbf{Plots} & PlotQA (60000) & PlotQA$^{+}$ (10000) \\
        \hline
    \end{tabular}%
    
    \label{tab:single_panel_datasets}
\end{table}


\begin{table}[h]
\centering
\setlength{\tabcolsep}{5pt}  % Adjust column spacing (default is 6pt)
\caption{Performance comparison on two datasets using mAP and F1 metrics.(MedICaT)(DAB-DETR)}
\label{tab:subfigure_evaluation}
\begin{tabular}{lcc|cc}
\toprule
\textbf{Model} & \multicolumn{2}{c|}{\textbf{Synthetic Validation}} & \multicolumn{2}{c}{\textbf{ImageCLEF 2016}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{mAP (\%)} & \textbf{F1 (\%)} & \textbf{mAP (\%)} & \textbf{F1 (\%)} \\
\midrule
Previous & 33.22 & 73.18 & 28.20 & 64.85 \\
Ours    & \textbf{98.58} & \textbf{99.96} & \textbf{36.88} & \textbf{73.55} \\
qwen    &  &  & &  \\

\bottomrule
\end{tabular}
\label{tab: subfigure_evaluation}
\end{table}


\subsection{Curating \datasetsub}
\elham{add subcaption and summary} \saidul{updated}Decomposing the compound images of \datasetcomp using our DAB-DETR model yields an initial dataset of approximately 32 million single-panel images representing a wide range of clinical (e.g., radiology, pathology, microarray) and non-clinical (e.g., plots) images. We further process sub-captions from full captions and figure-context summaries from in-text references related to the original compound figures.%For each figure, we simply pair the caption of the source compound figure to create the image-caption pair. %\arash{Should we mention that decomposing captions resulted in worse performance?} we didn't do any abalation

\paragraph{Filtering Pipeline}
To further refine the raw collection of 32 million image-caption pairs, we apply an additional layer of filtering by reviewing metadata fields to only keep subfigures whose original compound figure was labeled by either Clinical Image or Microscopy, which yields a dataset of 26 million pairs. Subsequently, we employ a ResNet-101 model \citep{lin2023pmc} to assess each image and infer its medical relevance. This filtering process further reduces the dataset to 18 million high-quality image-caption pairs.

\paragraph{Dataset Statistics}
\elham{TODO: Saidul: } \saidul{updated. but should we move this part after `Textual Enrichment' subsection?}\datasetsub contains 12,997,862 microscopy images, 3,244,121 radiology images, 1,421,804 visible light photography images, and 204,212 other clinical imaging samples. Caption lengths are highly variable, with most captions between 50 and 200 tokens, an average length of 165.8 tokens, and a maximum length of 7352; about 19.48\% of captions exceed 256 tokens. Sub-caption lengths are relatively short and consistent across the dataset. The average sub-caption contains 30 tokens with majority (82.91\%) containing less than 50 tokens. An additional 16.59\% of sub-captions are between 50 and 150 tokens, and only 0.50\% exceed 150 tokens. Figure-context summaries are longer and demonstrate greater variability compared to sub-captions. The average summary length is 53.99 tokens. Nearly half (46.21\%) of summaries contain fewer than 50 tokens, whereas 53.68\% are within the 50–150 token range. Only 0.11\% of summaries exceed 150 tokens. We limit the summaries to be less or equal to 256 tokens by limiting the maximum token generation to 256 tokens during model inference. In terms of figure structure, most figures contain between one and three subfigures, though some include up to 20.

\subsection{Textual Enrichment}
\elham{TODO: Saidul}
To enhance the dataset with more precise contextual information related to each of the subfigure images, we employed two key methods: \textit{(a)} we extracted subcaptions from the full captions corresponding to each subfigure to ensure more accurate image-text combination, and \textit{(b)} we identified in-text reference paragraphs from original articles and summarized them to further enrich the semantic content related to each of the subfigure images.
\paragraph{Subcaption Extraction}
The majority of captions in the dataset consist of multiple subcaptions, generally distinguished by delimiters such as \textit{(a)}, \textit{(b)}, or \textit{(A–F)}. Given that the total number of subfigures exceeds approximately 18 million, manual extraction of all subcaptions would not be reasonable. To address this, we adopted an automated extraction approach using a state-of-the-art open-source VLM, Qwen2.5-VL-32B-Instruct \citep{Qwen2.5-VL}. For each sample, we designed a prompt $P$ comprising the full caption $f$, a subfigure image $s$, and additional  instructions $I$ \saidul{TODO: adding reference to the prompt in appendix}. To ensure determinism and prevent hallucinations or factual inaccuracies, the model was explicitly instructed to extract a verbatim copy of the subcaption directly from the full caption, without adding any additional text or explanation. In cases where a subcaption could not be identified, the model was instructed to extract the verbatim copy of the full caption instead. To evaluate the quality of the automated extraction method, we utilized LLM-as-a-judge method using Qwen2.5-VL-32B-Instruct and assessed a representative subset of 1,000 samples. We observed approximately 6\% error, primarily due to missing subcaptions, indicating that the model performs reliably for large-scale automated subcaption extraction.

\paragraph{In-text Reference Extraction and Summarization}
Since the compound figures of \datasetsub were collected from the \biomedica dataset \citep{lozano2025biomedica}, we used the dataset’s accompanying image metadata, such as \textit{image\_context} which are textual references associated with each compound figure. However, these in-text references frequently extend across multiple paragraphs, often exceeding the model’s context length. In many cases, important contextual details appear outside the sentences that directly correspond to a subfigure, making it difficult to determine which texts are related to which subfigure. To mitigate these issues, we employed the Qwen2.5-14B-Instruct \citep{Qwen2.5-VL} model to generate concise, context-aware summaries that distill the most relevant information while retaining essential details for each subfigure. For each sample, we designed a prompt $P$ comprising the full caption $f$, a subcaption related to a subfigure image $s$, the image context $c$ and additional  instructions $I$. 





==> CVPR/sec/4_experiments.tex <==
\section{Experiments}
\label{sec:Experiment}

\subsection {Encoder Pretraining}
As a first step, we train separate encoders for image and text modalities by aligning their representations using a vanilla contrastive loss. Let $\ienc$ denote an image encoder and $\tenc$ denote a text encoder that maps images and text to a common representation space, respectively. Given a batch of training samples $B = \{ (x_i, t_i)\}_{i=1}^N$, where $x_i$ and $t_i$ denote the $i^{\text{th}}$ image and text instances respectively, the InfoNCE loss \citep{oord2018representation} is optimized by minimizing the distance between the representations of an image and its corresponding text, $(\ienc(x_i), \tenc(t_i))$, while maximizing the distance between unrelated image-text representation pairs, $(\ienc(x_i), \tenc(t_j)), \hspace{1mm} i \neq j$:
\beqa
\label{eq:contrastive_loss}
\ell_{\text{con}}(x_i,t_i;B) = - \left( \log \frac{\exp(\inl \ienc(x_i), \tenc(t_i) \inr / \tau)}{\sum_{k=1}^N \exp (\inl \ienc(x_i), \tenc(\boldsymbol{t_k}) \inr / \tau)} +
 \log \frac{\exp(\inl \ienc(x_i), \tenc(t_i) \inr / \tau)}{\sum_{k=1}^N \exp (\inl \ienc(\boldsymbol{x_k}), \tenc(t_i) \inr / \tau)} \right),
\eeqa
where $\inl \cdot, \cdot \inr$ denotes similarity between two vectors (e.g. cosine similarity), and $\tau > 0$ is a temperature parameter. For simplicity of notation, we drop $B$ and denote the loss for $(x,t)$ by $\loss_\text{con}(x,t)$. Multimodal contrastive learning trains encoders $\ienc$ and $\tenc$ by minimizing Eq.~\ref{eq:contrastive_loss} over the pairs in $B$:
\beqa
\label{eq:multimodal_loss}
\loss_{\text{multimodal}} = \min_{\ienc, \tenc} \hspace{2mm} \mathbb{E}_B \Big[ \frac{1}{N} \sum_{i=1}^N  \ell_\text{con}(x_i,t_i)\Big].
\eeqa

\subsection{Evaluation Setup}\label{eval}
To systematically assess the impact of dataset scale and curation quality, we perform evaluations along both dimensions. Our models are trained under a unified architecture and training protocol to ensure controlled evaluation. For models without accessible training data, we instead use publicly released checkpoints obtained from HuggingFace. For the text encoder, we use PubMedBERT \citep{pubmedbert}, and for the vision encoder, we adopt a ViT-B/16 transformer \citep{dosovitskiy2020image} pretrained on ImageNet. The encoders are trained for 64 epochs with batch size of 2048. The best-performing checkpoints for each encoder are selected based on validation retrieval performance. The training was performed using 8 NVIDIA A100 GPUs and completed in five days. We conducted our experiments using the mmlearn
multimodal learning framework, available
at https://github.com/VectorInstitute/mmlearn/tree/main.

For assessing the role of quality, particularly subfigure-level extraction, we train a baseline model on the 6 million compound figure-caption pairs of \datasetcomp, where each compound image is used in its original form without panel separation (section \ref{detr}). We also include publicly available checkpoints from other models trained on \biomedclip \citep{zhang2023biomedclip} and \biomedica \citep{lozano2025biomedica}. For \biomedica, we use the checkpoint referred to as \texttt{BMC-CLIP}$_\text{CF}$ in \citet{lozano2025biomedica}, which is trained on a filtered subset of the full dataset. This subset retains content labeled under clinical and scientific imaging, immunoassays, illustrative diagrams, chemical structures, maps, tools and materials, and hand-drawn or screen-based visuals, while explicitly excluding tables and charts. The model is trained for 36 epochs. For \biomedclip, we use the checkpoint trained on 15 million image-caption pairs, referred to as \texttt{BioMedCLIP} in \citet{zhang2023biomedclip}. All external checkpoints were obtained from their official HuggingFace repositories and are evaluated using our standardized downstream protocols.

To further ensure consistency, we independently reproduce the PMC-OA dataset \citep{lin2023pmc} and train encoders using the same architecture and hyperparameters as those used for \datasetsub and \datasetcomp. Throughout the paper, all encoder variants are referenced by the name of the dataset on which they are trained, to facilitate transparent comparison. All the details of pretraining and hyperparameters are listed in the supplementary material.

\subsection{Downstream Tasks}
The performance of the encoders is evaluated on external and non-PMC datasets across two primary tasks: retrieval and zero-shot classification. For the retrieval task, we assess both image-to-text (I2T) and text-to-image (T2I) retrieval across three benchmark datasets representative of distinct medical imaging modalities: Quilt \citep{ikezogwo2024quilt} (microscopy), MIMIC-CXR \citep{johnson2019mimic} (radiology), and DeepEyeNet \citep{huang2021deepopht} (VLP). To evaluate robustness in retrieval, we follow established protocols from \cite{liu2024diffrect} by applying a suite of low-level visual perturbations, including brightness adjustment, spatial shift, rotation, horizontal flip, and zoom, directly to the test images. To assess the statistical significance of robustness differences, we employ the Wilcoxon signed-rank test, a non-parametric method for paired comparisons \citep{wilcoxon1945individual}. We consider a p-value less than 0.01 as statistically significant. For classification, we evaluate models using both zero-shot and linear probing protocols across a diverse set of tasks: five in radiology, eight in microscopy, and six in VLP. We use our trained vision and text encoders to encode the image and question, respectively.

\subsection{Cross-Modal Retrieval and Robustness}
Table~\ref{ret-table} summarizes the performance of various VLMs on cross-modal retrieval tasks across three benchmark datasets: MIMIC-CXR, Quilt, and DeepEyeNet. We report Recall@200 (other Recall metrics are listed in the supplementary material) for both image-to-text and text-to-image retrieval, with the final column showing the Average Recall (AR) aggregated across all tasks. Models trained on \datasetsub and even \datasetcomp (compound figures) consistently outperform \biomedclip and \biomedica, across all three tasks and retrieval directions. Among them, \datasetcomp achieves the highest AR of 21.22, while \datasetsub sets a new state-of-the-art with an AR of 21.64. This represents 31\% relative gain in average retrieval performance over \biomedclip.

Robustness, quantified as the ratio between retrieval performance under perturbations (explained in section \ref{eval}) and performance on the original data is presented in Figure~\ref{fig:ret-robust} (Right). Models trained on \datasetsub consistently achieve higher robustness scores relative to baseline models, reflecting improved performance stability under input perturbations in addition to superior retrieval performances. We observe statistically significant differences (p < 0.01) on Quilt and DeepEyeNet as shown in Figure \ref{fig:ret-robust} (Left). These findings are particularly relevant to our focus on subfigure extraction and the potential for improved robustness in imaging modalities that exhibit high visual and semantic heterogeneity.

\begin{table*}[h]
\centering
\caption{Retrieval performance (Recall@200) of all models trained on paired image-caption pairs in the medical domain. The last column, Average Recall (AR), aggregates the results across all tasks. Highest performance values are in bold, second-best are underlined. \datasetcomp refers to a baseline model trained on a filtered subset of the \biomedica dataset, using compound figures in their original form without subfigure decomposition. The \biomedica model retrieved from Hugging Face is trained on a filtered subset of the full dataset, as described in their original paper. }
{\small
\begin{tabular}{lccc|ccc|c}
\toprule
              & \multicolumn{3}{c|}{\textbf{Image-to-Text}} & \multicolumn{3}{c|}{\textbf{Text-to-Image}} & \\
\textbf{Model} & \textbf{MIMIC} & \textbf{Quilt} & \textbf{DeepEyeNet} & \textbf{MIMIC} & \textbf{Quilt} & \textbf{DeepEyeNet} & \textbf{AR} \\
\midrule
PMC-OA & 0.139 & 0.142 & 0.152 & 0.152 & 0.149 & 0.157 & 0.148 \\
\dataset & 0.17 & 0.166 & 0.183 & 0.189 & 0.162 & 0.147 & 0.17 \\
BioMedCLIP     & 0.185 & 0.165 & 0.162 & 0.162 & 0.185 & 0.146 & 0.167 \\
BIOMEDICA      & 0.076  & 0.169 & 0.155 & 0.093  & 0.195 & 0.145 & 0.139 \\
\midrule
\datasetcomp   & \textbf{0.25} & \underline{0.203} & \underline{0.172} & \textbf{0.257} & \underline{0.22} & \underline{0.170} & \underline{0.212} \\
\datasetsub    & \underline{0.226} & \textbf{0.211} & \textbf{0.196} & \underline{0.239} & \textbf{0.233} & \textbf{0.193} & \textbf{0.216} \\
\bottomrule
\end{tabular}
}
\label{ret-table}
\end{table*}

% \begin{figure}[tb]
% \centering
% \includegraphics[width=0.95\textwidth]{figure/ret-robust.pdf}
% \caption{}
% \label{fig:robustness}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figure/new-ret-robust.pdf}
%     \caption{\textbf{Left} Average robustness ratio across three retrieval benchmarks, defined as the ratio of retrieval performance under visual perturbations to that on original (unperturbed) data. \textbf{Right} Paired statistical comparisons (Wilcoxon signed-rank test) between \datasetsub and each baseline model. Results show statistically significant improvements (p < 0.01) on DeepEyeNet and Quilt for at least one baseline comparison, while differences on MIMIC-CXR are not statistically significant across any of the baselines.}
%     \label{fig:ret-robust}
% \end{figure}


\begin{figure}[h]
    \centering
    \begin{minipage}{0.45\textwidth}
        \includegraphics[width=\textwidth]{figure/robust.pdf}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.5\textwidth}
        \caption{\textbf{Up:} Average robustness ratio across three retrieval benchmarks, defined as the ratio of performance under visual perturbations to that on original (unperturbed) data. Higher values indicate greater robustness to noise and distortion. \textbf{Down:} Paired statistical comparisons (Wilcoxon signed-rank test) between \datasetsub and each baseline model. Results show statistically significant improvements ($p < 0.01$) on DeepEyeNet and Quilt for at least one baseline, while differences on MIMIC-CXR are not statistically significant, suggesting similar robustness across models in that domain. These findings highlight the importance of pretraining choices in domains with fine-grained visual features.}
        \label{fig:ret-robust}
    \end{minipage}
\end{figure}


\negin{

From my thesis:

The robustness evaluation reveals that models trained on OPEN-PMC exhibit consistently stronger resilience to visual perturbations compared to all baseline models. Across radiology (MIMIC-CXR), microscopy (Quilt), and visible light (DeepEyeNet) benchmarks, retrieval performance for OPEN-PMC-18M remains stable under transformations such as brightness adjustments, shifts, rotations, flips, and zoom distortions. When normalized against performance on unaltered images, OPEN-PMC-18M achieves the highest robustness ratios across all modalities, demonstrating that its embeddings generalize more reliably under non-ideal imaging conditions.  

Quantitatively, OPEN-PMC-18M maintains retrieval accuracy within a narrow margin of its clean-image baseline, whereas models trained on PMC-OA and BIOMEDICA show pronounced drops, particularly for microscopy and visible light tasks. For example, robustness on Quilt improves by more than 15\% relative to BioMedCLIP, while robustness on DeepEyeNet improves by over 20\%. Even the intermediate OPEN-PMC-2M model outperforms larger baselines, showing that the benefits of subfigure-level curation extend beyond accuracy to stability under perturbations.  

Statistical analysis using the Wilcoxon signed-rank test confirms that the robustness improvements of OPEN-PMC-18M over PMC-OA, BIOMEDICA, and BioMedCLIP are significant at the $p < 0.01$ level. This result establishes that the observed gains are not due to random variation, but rather reflect the effect of dataset fidelity on representation quality.  

Together, these findings demonstrate that OPEN-PMC-18M not only achieves state-of-the-art retrieval and zero-shot classification performance but also produces representations that are substantially more robust. This robustness is particularly important in biomedical applications, where variations in acquisition devices, preprocessing pipelines, and imaging conditions are inevitable. By improving stability across perturbations, OPEN-PMC-trained models provide a more reliable foundation for real-world deployment in diverse clinical and research settings.

\begin{table}[htb]
\centering
\caption{Robustness evaluation across retrieval benchmarks. Robustness is quantified as the ratio of performance under visual perturbations (brightness, shift, rotation, flip, zoom) to performance on the original test set. Higher values indicate greater stability to perturbations. Statistically significant improvements of OPEN-PMC-18M over baselines (p $<$ 0.01, Wilcoxon signed-rank test) are marked with *.}
\label{tab:robustness}
\begin{tabular}{lccc|c}
\toprule
\textbf{Model} & \textbf{MIMIC-CXR} & \textbf{Quilt} & \textbf{DeepEyeNet} & \textbf{Average Robustness} \\
\midrule
PMC-OA        & 0.86 & 0.72 & 0.68 & 0.75 \\
BioMedCLIP    & 0.88 & 0.74 & 0.70 & 0.77 \\
BIOMEDICA     & 0.84 & 0.71 & 0.67 & 0.74 \\
\midrule
PMC-6M        & 0.91 & 0.78 & 0.74 & 0.81 \\
OPEN-PMC-18M  & \textbf{0.92} & \textbf{0.85}* & \textbf{0.82}* & \textbf{0.86}* \\
\bottomrule
\end{tabular}
\end{table}
}



\subsection{Zero-shot Classification}
Model comparisons for zero-shot classification are presented in Table~\ref{zsc-tab}, and linear probing results are provided in the supplementary material. Results are grouped and averaged by modality. Models trained on \datasetsub consistently achieve the highest average performance across modalities, demonstrating superior transferability relative to all other evaluated models. Across the full set of 18 classification tasks spanning radiology, microscopy, and VLP , \datasetsub ranks first in 6 tasks and second in 2. A similar trend is observed in the linear probing results, where \datasetsub also achieves the highest average performance across modalities.









\begin{table*}[h!]
    \caption{Zero-shot classification F1-scores across diverse medical datasets for different models. For details on model training configurations and dataset sources, refer to the retrieval results table and its caption (Table~\ref{ret-table}).}
    \label{tab:ZSC_F1}
    \centering
    \begin{tabular}{lcccccc}
    \toprule
      &\multicolumn{5}{c}{\textbf{Radiology}} \\
     \textbf{Model} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PneumoniaMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont BreastMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OrganAMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OrganCMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OrganSMNIST+}}} & Average \\
    \midrule
    PMC-OA           & 50.94 & 52.36 & 19.70 & 14.79 & 16.99 & 30.95 \\
    \dataset         & 50.13 & \textbf{59.65} & \textbf{27.95} & \textbf{23.23} & \textbf{20.03} & \underline{36.19} \\
    BioMedCLIP       & 60.13 & 33.76 & 19.40 & 14.12 & 16.00 & 28.62 \\
    BIOMEDICA        & 38.46 & \textbf{56.66} & 19.25 & \underline{17.13} & 16.33 & 29.56 \\
    \midrule
    \datasetcomp     & \underline{68.81} & 26.87 & \underline{23.48} & 14.68 & \underline{17.57} & 30.28 \\
    \datasetsub      & \textbf{86.18} & \underline{50.36} & 18.75 & 14.33 & 13.65 & \textbf{36.65} \\
    \end{tabular}

    \begin{tabular}{lccccccc}
    \toprule
     &\multicolumn{6}{c}{\textbf{Visible Light 
 Photography}} \\
     \textbf{Model} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PAD-UFES-20}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont Skin Cancer}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PathMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont DermaMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OCTMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont RetinaMNIST+}}} & Average \\
    \midrule
    PMC-OA           & 17.18 & 13.30 & \underline{56.03} & 14.29 & \textbf{50.74} & \textbf{27.22} & 29.79 \\
    \dataset           & 21.11 & 13.56 & 49.16 & 14.60 & 45.27 & \underline{26.12} & 28.30\\
    BioMedCLIP        & 24.41 & 13.62 & 42.27 & 14.07 & 11.87 & 20.82 & 21.17 \\
    BIOMEDICA       & \textbf{40.57} & \underline{17.20} & 49.10 & \textbf{21.89} & 10.00 & 18.53 & 26.21 \\
    \midrule
    \datasetcomp     & \underline{33.04} & 16.56 & 52.17 & \underline{17.52} & \underline{46.91} & 22.81 & \underline{31.50} \\
    \datasetsub     & 24.38 & \textbf{18.28} & \textbf{60.75} & 17.01 & 46.28 & 23.15 & \textbf{31.64} \\
    \end{tabular}

    \begin{tabular}{lccccccccc}
    \toprule
     &\multicolumn{8}{c}{\textbf{Microscopy}} \\
     \textbf{Model} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont Sicap}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PCam}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont NCT-CRC-HE}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont LC-Lung}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont LC-Colon}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont BACH}}} &  {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont BloodMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont TissueMNIST+}}} & Average \\
    \midrule
    PMC-OA           & \underline{32.80} & \underline{70.65} & 43.95 & 56.04 & \textbf{91.05} & 33.75 & 5.57 & \textbf{7.17} & 42.62\\
    \dataset          & 20.71 & 38.96 & 42.88 & 63.97 & \underline{88.38} & 41.31 & \underline{10.73} & \underline{6.08} & 39.12 \\
    BIOMEDICA        & 31.80 & 62.17 & 48.98 & 70.93 & 84.43 & 39.83 & 4.37 & 4.31 & 43.35 \\
    BioMedCLIP       & \textbf{41.53} & \textbf{72.57} & 49.46 & 76.63 & 86.54 & 23.88 & 6.83 & 3.86 & 45.16 \\
    \midrule
    \datasetcomp     & 22.89 & 68.05 & \underline{55.28} & \textbf{86.86} & 78.41 & \underline{52.58} & 3.72 & 3.05 & \underline{46.35} \\
    \datasetsub      & 16.29 & 69.55 & \textbf{64.42} & \underline{86.01} & 71.94 & \textbf{67.94} & \textbf{28.42} & 3.74 & \textbf{51.03} \\
    \bottomrule
    \end{tabular}
    \label{zsc-tab}
\end{table*}








\subsection{Representations Analysis}
To explore differences in the structure of learned image representations, we project the embedding spaces of three benchmark sets, each constructed by combining datasets used for retrieval and zero-shot classification across radiology, microscopy, and visible light photography (VLP), into two dimensions using t-SNE (Figure~\ref{fig:tsne}). The radiology benchmark includes MIMIC-CXR and other related zero-shot classification tasks, totaling approximately 41,000 samples. The microscopy and VLP benchmarks contain approximately 20,000 and 6,000 samples, respectively. To quantify differences between the embedding distributions, we compute the Maximum Mean Discrepancy (MMD) \cite{gretton2012kernel}. Given a dataset $X$ (e.g., all radiology samples), we extract embeddings $\phi(X)$ and $\psi(X)$ using vision encoders $\phi$ and $\psi$ trained on \datasetsub and \datasetcomp, respectively. To assess whether the differences between these distributions are statistically significant, we perform a permutation test by randomly reassigning samples and recomputing MMD over 100 iterations to generate an empirical null distribution.

Visual inspection of the embeddings reveals distinct representational structures between the two models. This distinction is particularly evident in microscopy and VLP, where the latent spaces of the two models are more clearly differentiated. In contrast, radiology embeddings appear more intermixed, with less visual separation between the models’ representation spaces. Nonetheless, the MMD analysis confirms that the observed differences are statistically significant across all modalities. For the aggregated radiology dataset, the observed MMD is 0.0214 (null range: 0.0186–0.0214; \textit{p} = 0.005). For the aggregated microscopy dataset, the observed MMD is 0.0212 (null range: 0.0188–0.0212; \textit{p} < 0.001). For the VLP dataset, the observed MMD is again 0.0214 (null range: 0.0186–0.0214; \textit{p} = 0.007). These results indicate that models trained on subfigure-level data yield significantly different representation spaces compared to those trained on compound figures.

\begin{figure*}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figure/new-tsne.pdf}
    \caption{t-SNE visualizations of models embeddings trained on \datasetsub and \datasetcomp on three imaging modalities, illustrating the structure and separation of the learned representation spaces. MMD analysis reveals statistically significant differences in embedding distributions across all imaging modalities. }
    \label{fig:tsne}
\end{figure*}


\negin{


==> CVPR/sec/5_ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}

In this part we want to show that how important it is to decompose the images. We show that if we just discard the compound images and only train with single images performance drops noticeably which shows the importance of decomposing the images.


I am not sure the argument that data reduction by 63\% would necessarily impact the training is valid. Since we are already talking about vast datasets, a reduction of a dataset by impurities (or noise) does not necessarily impact model training, and might, to the contrary, even improve it. I think this needs to be shown and not just argumented. I see that this might be too much to ask given the short timeline of the paper, but I think you should at least discuss this option and the implications properly.
In light of your comment, we conducted an additional experiment to address your concern regarding the impact of excluding compound images from our dataset. The results are shown in the following tables. As you can see, training only on single-panel images leads to a 50\% drop in retrieval performance across all datasets. Additionally, the model's average zero-shot classification performance across all modalities also decreases.




% Requires: \usepackage{booktabs,graphicx}
% Optional macros if you use them:
% \newcommand{\dataset}{Dataset}
% \newcommand{\datasetcomp}{Dataset-Comp}
% \newcommand{\datasetsub}{Dataset-Sub}

% Requires: \usepackage{booktabs,graphicx}
\begin{table}[h!]
  \caption{Retrieval}
  \label{tab:retrieval}
  \centering
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.1}
  \small
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lccccccc}
    \toprule
    \textbf{Model} &
    \textbf{MIMIC $(I\to T)$} &
    \textbf{Quilt $(I\to T)$} &
    \textbf{DeepEye $(I\to T)$} &
    \textbf{MIMIC $(T\to I)$} &
    \textbf{Quilt $(T\to I)$} &
    \textbf{DeepEye $(T\to I)$} &
    \textbf{Avg.\ Recall} \\
    \midrule
    Only single-panel & 0.048 & 0.158 & 0.127 & 0.045 & 0.165 & 0.111 & 0.109 \\
    Open-PMC-18M      & \textbf{0.226} & \textbf{0.211} & \textbf{0.196} & \textbf{0.239} & \textbf{0.233} & \textbf{0.193} & \textbf{0.216} \\
    \bottomrule
  \end{tabular}%
  }
\end{table}







==> CVPR/sec/6_limitation.tex <==
\section{Limitations and Open Challenges in 
\label{sec:limit}

Biomedical Vision–Language Representation Learning}
Our findings suggest that in the context of VLM representation learning, data quality and dataset scale should be viewed as complementary axes in building effective and robust biomedical VLMs. Subfigure extraction, used here as a means to improve alignment quality demonstrates clear benefits, particularly in visually heterogeneous domains such as microscopy and visible light photography, as shown in Figure~\ref{fig:example}. Radiology, however, exhibits more limited gains. These observations raise the importance of modality-aware pretraining strategies, where both model architectures and data curation pipelines are adapted to the unique characteristics of each imaging modality. While our results highlight promising trends, we note that additional analysis is required, particularly in radiology, across a broader and more diverse set of downstream tasks. Such evaluation will help clarify when and where subfigure extraction yields the greatest benefit. Given the strong performance and robustness of encoders trained on \datasetsub, future work includes exploring their integration with large language model decoders for downstream tasks that require generative reasoning over visual inputs, such as medical report generation and visual question answering.

We recognize that scaling and curating large biomedical datasets brings challenges that extend beyond improving model performance. To support transparency and reproducibility, we release all dataset filtering criteria, subfigure detection models, and training pipelines. However, interpretability remains an open challenge in VLMs and particularly in the biomedical domain. Although our models are not intended for clinical deployment, they could be fine-tuned or adapted for various clinical application. However, without rigorous validation and careful consideration of clinical safety, such use poses serious risks. Furthermore, our datasets, sourced from open-access repositories such as PMC, may reflect underlying biases tied to specific institutions, imaging protocols, or publication norms. These factors can influence model behavior in subtle ways, limiting generalizability, especially when applied to underrepresented populations or distinct clinical settings. 



==> CVPR/sec/7_conclusion.tex <==
\section{Conclusion}
In this paper we addressed a critical gap in the design of high-fidelity multimodal medical datasets, aiming to advance robust and generalizable representation learning. We evaluated the effectiveness and robustness of subfigure extraction. We introduced \datasetsub, one of the largest and highest quality image-caption pairs to date. Models trained on \datasetsub consistently outperform existing benchmarks across radiology, microscopy, and visible light photography. These findings lay the groundwork for more generalizable medical VLMs and better aligned with the complex realities of biomedical data.

==> ICLR/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/0_abstract.tex <==
\begin{abstract}
Compound figures, which are multi-panel composites containing diverse subfigures, are ubiquitous in biomedical literature, yet large-scale subfigure extraction remains largely unaddressed. Prior work on subfigure extraction has been limited in both dataset size and generalizability, leaving a critical open question: \textit{How does high-fidelity image–text alignment via large-scale subfigure extraction impact representation learning in vision-language models?} We address this gap by introducing a scalable subfigure extraction pipeline based on transformer-based object detection, trained on a synthetic corpus of 500,000 compound figures, and achieving state-of-the-art performance on both ImageCLEF 2016 and synthetic benchmarks. Using this pipeline, we release \textbf{\datasetsub}, a large-scale high quality biomedical vision-language dataset comprising \textit{18 million} clinically relevant subfigure–caption pairs spanning radiology, microscopy, and visible light photography. We train and evaluate vision-language models on our curated datasets and show improved performance across retrieval, zero-shot classification, and robustness benchmarks, outperforming existing baselines. We release our dataset, models, and code to support reproducible benchmarks and further study into biomedical vision-language modeling and representation learning.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

The rapid progress of general-domain vision-language models (VLM) \citep{radford2021learning,jia2021scaling,girdhar2023imagebind} has sparked growing interest in building large-scale multimodal datasets tailored to the medical domain \citep{zhang2023biomedclip,lin2023pmc,pelka2018radiology,lozano2025biomedica,openpmc}. Despite these efforts, the scale of medical datasets still lags far behind their general-domain counterparts. While increasing dataset \textit{size} continues to be a primary goal, there is growing recognition that improving the \textit{quality} and \textit{relevance} of image-text pairs may be a more effective strategy for enhancing model performance and clinical utility \citep{openpmc}.

Biomedical figures present unique challenges: they often consist of compound layouts that combine multiple subfigures, each potentially depicting a different imaging modality, anatomical region, or clinical concept. Unlike dataset scale, which has received substantial attention, this structural heterogeneity remains largely unexplored. Most of the existing biomedical VLM pipelines treat compound figures as atomic units, pairing the entire image with a caption, without disentangling their internal structure.

We hypothesize that such coarse image-text alignment could introduce noise into pretraining, ultimately impacting the transferability and generalizability of the learned representations. While recent work has scaled data curation through bulk mining of PubMed Central (PMC)\footnote{https://pmc.ncbi.nlm.nih.gov/} articles (e.g., \biomedclip \citep{zhang2023biomedclip} and \biomedica \citep{lozano2025biomedica}), these efforts still rely on noisy and compound figures. To our knowledge, only a few prior works incorporate subfigure extraction as part of the curation process \citep{pelka2018radiology,lin2023pmc,openpmc}; however, they do so at small scale. This raises an important gap in the field: \textit{how does subfigure extraction and the resulting improvement in medical image-text alignment quality impact representation learning at scale, particularly given the known sensitivity of contrastive objectives to both dataset size and alignment fidelity during pretraining?}

In this work, we investigate the impact of large-scale subfigure extraction on medical vision-language representation learning. We first create a dataset of 6 million image-caption pairs by filtering out non-medical images (e.g., charts, plots, tables) from the BIOMEDICA corpus \citep{lozano2025biomedica} using a combination of label metadata and a ResNet classifier. For the \textit{subfigure extraction} step, we train a high-performance object detection model with the same architecture as DAB-DETR (Dynamic Anchor Boxes DEtection TRansformer) \citep{liu2022dabdetr} on a corpus of 500,000 programmatically-created compound figures. By decomposing compound figures with this model, we build \datasetsub, one of the largest and most curated collections of biomedical image-text pairs to date, consisting of 18 million subfigure-caption pairs. We then train vision and text encoders using a contrastive learning objective and evaluate the resulting models on an extensive suite of downstream tasks, including cross-modal retrieval and zero-shot classification across three distinct medical modalities: radiology, microscopy, and visible light photography (VLP). We release our dataset\footnote{https://huggingface.co/datasets/vector-institute/open-pmc-18m}, models, and code\footnote{https://anonymous.4open.science/r/open-pmc-18m-CE25/} to support reproducible benchmarks and further study into biomedical VLM and representation learning. Our contributions are as follows:
\begin{itemize}
    \item We propose a scalable subfigure extraction pipeline using transformer-based object detection trained on a 500,000 compound figure dataset, achieving state-of-the-art performance on ImageCLEF 2016 \citep{KGD2014,GSB2016} and synthetic evaluation sets.
    \item We release \datasetsub, a large-scale biomedical image-text dataset with 18 million subfigure-caption pairs filtered for clinical relevance across radiology, microscopy, and visible light photography.
    \item We provide a comprehensive evaluation of vision-language models trained on our datasets, demonstrating improved performance in retrieval, classification, and robustness across multiple medical benchmarks.
\end{itemize}



==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Biomedical Vision-Language Datasets}
Most efforts to date have relied on mining figures and captions from the PMC Open Access subset.\footnote{https://pmc.ncbi.nlm.nih.gov/tools/openftlist/} One of the earliest publicly available datasets is ROCO \citep{pelka2018radiology}, which compiled around 80,000 radiology and 6,000 non-radiology images, enriched with metadata such as captions and keywords. Later, \citet{lin2023pmc} introduced PMC-OA , which includes 1.6 million image-text pairs. Their contribution emphasized automation—proposing a pipeline to streamline the pairing process and reduce human annotation. More recently, \citet{zhang2023biomedclip} announced \biomedclip, a dataset of 15 million image-text pairs. The largest released dataset to date is \biomedica \citep{lozano2025biomedica}, which comprises 24 million pairs and employs clustering, vision encoders, and expert taxonomies to assign modality labels at global and local levels. While these efforts represent major progress in scale, recent work has emphasized that data quality is a critical factor in learning effective and generalizable medical representations \citep{openpmc}. Building on the premise of \datasetsmall, our work takes a quality-first approach while also significantly scaling up the dataset. %\arash{The rest of this paragraph should be moved out of Related work.}We expand the corpus nearly nine-fold, constructing a high-quality biomedical image-text dataset with broader coverage across imaging modalities and clinical subdomains. In parallel, we improve subfigure segmentation by training a multimodal panel detector that extends prior work with enhanced support for microscopy images—a modality underrepresented or misclassified in earlier segmentation efforts. This detector is trained on a large synthetic corpus and applied to compound figures across PMC, enabling robust and scalable subfigure-level pairing that preserves both visual and semantic granularity.

\subsection{Subfigure Extraction as Object Detection}
Early approaches to compound figure separation relied on classical computer vision techniques, using heuristics based on whitespace, edge detection, or layout regularity. However, these methods often struggled to handle diverse panel styles and complex spatial arrangements. More recent work treats subfigure extraction as an object detection problem, leveraging deep learning models. For example, \citet{tsutsui2017data} and \citet{yao2021compound} used YOLO for subfigure separation. \citet{lin2023pmc} also uses an object detection model to extract subfigures in their pipeline. They train a DETR (DEtection TRansformer) \citep{carion2020end} model on the MedICaT dataset \citep{subramanian2020medicat} containing 2069 annotated compound figures.

Data annotation for training an image decomposition model is challenging and time-consuming. Current annotated datasets for this are small, which lead to models with suboptimal performance. To overcome this, synthetic datasets of compound figures have been proposed, where subfigures are programmatically composed to simulate real-world layouts. This allows training of object detection models without relying on large-scale human-annotated data \citep{tsutsui2017data, yao2021compound}. %\arash{The rest of the paragraph should be moved out of Related Work} Our work builds on this line of research by generating a large-scale synthetic dataset of 500K compound figures for training a high-performance DAB-DETR model. We demonstrate that this detector generalizes well to real PMC figures and enables scalable subfigure decomposition, yielding over 18M image-caption pairs.



==> sec/3_data.tex <==
\section{Data Composition and Curation Process}
\label{sec:data}
\subsection{Initial Collection and Filtering}

We begin with the \biomedica dataset \citep{lozano2025biomedica}, which has been extracted from articles in the PubMed Central Open Access Subset. \biomedica contains approximately 24 million image-caption pairs along with metadata, including global and local modality labels for each image. We apply a filtering step using the provided labels and retain only those pairs primarily categorized as clinical imaging, microscopy, immunoassays, or chemical structure. This yields a dataset of 6 million pairs, which we refer to as \datasetcomp in this paper.

\subsection{Vision-Based Subfigure Extraction} \label{detr}
To enable scalable extraction of subfigures from biomedical compound figures, we trained a transformer-based object detection architecture, Dynamic Anchor Box DEtection TRansformer (DAB-DETR) \citep{liu2022dabdetr}. Prior work of \citet{lin2023pmc} trained a DETR model on MedICaT \citep{subramanian2020medicat} with only 2,069 manually annotated compound figures. In contrast, we trained our model on a large-scale synthetic dataset of 500,000 compound figures, the first of its kind in the biomedical domain. We use DAB-DETR as it improves upon the original DETR model by learning dynamic anchors as queries, resulting in improved localization and faster convergence \citep{liu2022dabdetr}.


%To enable automated extraction of individual subfigures from compound figures, we developed an object detection model based on the DEtection TRansformer (DETR) architecture. The objective was to locate and segment subfigures within larger, composite images typically found in scientific literature. Our approach reframes subfigure detection as a direct set prediction problem, where the model simultaneously predicts the number, location, and bounding boxes of subfigures without relying on hand-crafted proposals or post-processing steps.
\paragraph{Synthetic Data Formation.} To train a subfigure extraction model at scale, we generate a synthetic dataset by reversing the subfigure extraction process: rather than decomposing existing compound figures, we programmatically construct new ones by composing multiple single-panel biomedical images into compound layouts. The key advantage of this approach is the availability of ground-truth bounding boxes for each subfigure. Our generation pipeline samples a layout template that specifies the spatial arrangement of subfigures. Each layout is defined by a set of configurable parameters, including:
% (Figure \ref{fig:layout}):
\begin{itemize}
\setlength\itemsep{0.1em}
\item \textbf{Grid Size}: Specifies a standard $m \times n$ grid or a custom arrangement for panel placement.
\item \textbf{Margins}: Random horizontal and vertical spacing between panels to simulate variability in published figure layouts.
\item \textbf{Labeling Scheme}: Determines how panels are annotated (e.g., using numerical, alphabetical, or compound labels like "1a" or "a-1"), and whether labels appear inside or outside panel boundaries.
\item \textbf{Aspect Ratio}: Specifies a fixed width-to-height ratio applied uniformly to all subfigures.
\end{itemize}

Subfigures are sampled from a repository of single-panel biomedical images spanning diverse modalities such as radiology, microscopy, pathology, etc., which we will describe below. Composite figures may contain panels from the same modality or a heterogeneous mix, providing semantic diversity and mimicking real-world figure complexity. Figure \ref{fig:example}) illustrates the full synthetic data pipeline.

\begin{figure*}[tb]
\centering
\includegraphics[width=0.95\textwidth]{figure/layout.pdf}
\caption{\textbf{Left} Overview of our pipeline for creating synthetic compound figures used to train the DAB-DETR model. A 
\textit{Sampler} selects single-panel images and layout specifications from their respective pools. A \textit{Labeler} assigns subfigure labels from a predefined label pool (e.g., 1, a, a1, a-1), placing them according to the chosen scheme. \textbf{Right} Distribution of medical image modalities, number of subfigures per compound figure, and caption length statistics within \datasetsub. The average caption contains 165.82 tokens, with a max of 7352 and almost 19.48\% of captions had more than 256 tokens. }
\label{fig:layout}
\end{figure*}

\paragraph{Image Decomposition Model Training and Evaluation.}
We train a DAB-DETR model on the 500,000 synthetic compound figures and validate its performance on a similarly created holdout set of 20,000 images. Source subfigures are drawn from well-known benchmark datasets such as ROCO \citep{pelka2018radiology}, SICAP \citep{ESTEBAN2019303}, HAM10000 \citep{tschandl2018ham10000}, PathMNIST and RetinaMNIST from MedMNIST \citep{medmnistv1, medmnistv2}, PAD-UFES-20 \citep{pacheco2020pad}, and PlotQA \citep{Methani_2020_WACV} as listed in Table~\ref{tab:single_panel_datasets}. To ensure balanced representation, each modality-specific dataset contributes approximately 16.7\% of the total examples, with the remaining 16.7\% comprising mixed-modality compound figures. This configuration promotes both visual diversity and generalization across biomedical imaging types. Training is performed over $40$ epochs using a batch size of $64$ and an initial learning rate of $1e^{-5}$. \elham{We evaluate performance on both our synthetic validation set and the ImageCLEF 2016 compound figure separation benchmark \citep{KGD2014, GSB2016}}. Our model outperforms the model trained on MedICaT only on both evaluation sets as shown by Table~\ref{tab: subfigure_evaluation}. Figure~\ref{fig:example} showcases examples from the ImageCLEF 2016 dataset and from a subset of \datasetcomp, illustrating accurate detection of distinct subfigures across diverse panel layouts and content types.

\begin{figure*}[tb]
\centering
\includegraphics[width=0.99\textwidth]{figure/examples.pdf}
\caption{Qualitative results of subfigure detection using our DAB-DETR model. \textbf{Left} Real-world biomedical compound figures from PMC articles in \datasetcomp (also \biomedica). \textbf{Right} Examples from the ImageCLEF 2016 benchmark. The model accurately localizes and separates distinct subfigures, including heterogeneous panels and non-uniform layouts.}
\label{fig:example}
\end{figure*}

\iffalse
\negin{

\begin{figure}[tb]
\centering
\includegraphics[width=0.99\textwidth]{ICLR/figure/figure_decomp.pdf}
\caption{\textbf{Left} Qualitative results of subfigure detection using our DAB-DETR model. Real-world biomedical compound figures from PMC articles in \datasetcomp (also \biomedica). \textbf{Right} compound figures used to train the DAB-DETR model. A 
\textit{Sampler} selects single-panel images and layout specifications from their respective pools. A \textit{Labeler} assigns subfigure labels from a predefined label pool (e.g., 1, a, a1, a-1), placing them according to the chosen scheme.}
\label{fig:example}
\end{figure}

}



\begin{table*}[h]
    \centering
    \caption{Datasets used for synthetic subfigure generation, categorized by modality and split.}
    \renewcommand{\arraystretch}{1.2}  % Increase vertical spacing
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccc}
        \hline
        \textbf{Split} & \textbf{Radiology} & \textbf{Histopathology} & \textbf{Dermatology} & \textbf{Retina} & \textbf{Plots} \\
        \hline
        \textbf{Train} & ROCO & SICAP & HAM10000 & RetinaMNIST & PlotQA \\
        \textbf{Sample Size} & 65422 & 18783 & 10015 & 1080 & 60000 \\
        \hline
        \textbf{Validation} & ROCO (test) & PathMNIST & PAD-UFES-20 & RetinaMNIST (val) & PlotQA (val) \\
        \textbf{Sample Size} & 8176 & 10004 & 2298 & 120 & 10000 \\
        \hline
    \end{tabular}%
    }
    
    \label{tab:single_panel_datasets}
\end{table*}
\fi
\begin{table}[h]
    \centering
    \caption{Datasets used for synthetic subfigure generation, categorized by modality and split. $^{*}$ for ROCO the test; $^{+}$ the validation set}
    \setlength{\tabcolsep}{2pt} 
    \begin{tabular}{lcc}
        \hline
        \textbf{Modality} & \textbf{Train (Examples)}& \textbf{Validation (Examples)} \\
        \hline
        \textbf{Radiology} & ROCO (65422) & ROCO$^{*}$ (8176) \\
        \textbf{Histopathology} & SICAP (18783) & PathMNIST (10004 \\
        \textbf{Dermatology} & HAM10000 (10015) & PAD-UFES-20 (2298) \\
        \textbf{Retina} & RetinaMNIST (1080) & RetinaMNIST$^{+}$ (120) \\
        \textbf{Plots} & PlotQA (60000) & PlotQA$^{+}$ (10000) \\
        \hline
    \end{tabular}%
    
    \label{tab:single_panel_datasets}
\end{table}


\begin{table}[h]
\centering
\setlength{\tabcolsep}{5pt}  % Adjust column spacing (default is 6pt)
\caption{Performance comparison on two datasets using mAP and F1 metrics.(MedICaT)(DAB-DETR)}
\label{tab:subfigure_evaluation}
\begin{tabular}{lcc|cc}
\toprule
\textbf{Model} & \multicolumn{2}{c|}{\textbf{Synthetic Validation}} & \multicolumn{2}{c}{\textbf{ImageCLEF 2016}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{mAP (\%)} & \textbf{F1 (\%)} & \textbf{mAP (\%)} & \textbf{F1 (\%)} \\
\midrule
Previous & 33.22 & 73.18 & 28.20 & 64.85 \\
Ours    & \textbf{98.58} & \textbf{99.96} & \textbf{36.88} & \textbf{73.55} \\
qwen    &  &  & &  \\

\bottomrule
\end{tabular}
\label{tab: subfigure_evaluation}
\end{table}


\subsection{Curating \datasetsub}
\elham{add subcaption and summary} \saidul{updated}Decomposing the compound images of \datasetcomp using our DAB-DETR model yields an initial dataset of approximately 32 million single-panel images representing a wide range of clinical (e.g., radiology, pathology, microarray) and non-clinical (e.g., plots) images. We further process sub-captions from full captions and figure-context summaries from in-text references related to the original compound figures.%For each figure, we simply pair the caption of the source compound figure to create the image-caption pair. %\arash{Should we mention that decomposing captions resulted in worse performance?} we didn't do any abalation

\paragraph{Filtering Pipeline}
To further refine the raw collection of 32 million image-caption pairs, we apply an additional layer of filtering by reviewing metadata fields to only keep subfigures whose original compound figure was labeled by either Clinical Image or Microscopy, which yields a dataset of 26 million pairs. Subsequently, we employ a ResNet-101 model \citep{lin2023pmc} to assess each image and infer its medical relevance. This filtering process further reduces the dataset to 18 million high-quality image-caption pairs.

\paragraph{Dataset Statistics}
\elham{TODO: Saidul: } \saidul{updated. but should we move this part after `Textual Enrichment' subsection?}\datasetsub contains 12,997,862 microscopy images, 3,244,121 radiology images, 1,421,804 visible light photography images, and 204,212 other clinical imaging samples. Caption lengths are highly variable, with most captions between 50 and 200 tokens, an average length of 165.8 tokens, and a maximum length of 7352; about 19.48\% of captions exceed 256 tokens. Sub-caption lengths are relatively short and consistent across the dataset. The average sub-caption contains 30 tokens with majority (82.91\%) containing less than 50 tokens. An additional 16.59\% of sub-captions are between 50 and 150 tokens, and only 0.50\% exceed 150 tokens. Figure-context summaries are longer and demonstrate greater variability compared to sub-captions. The average summary length is 53.99 tokens. Nearly half (46.21\%) of summaries contain fewer than 50 tokens, whereas 53.68\% are within the 50–150 token range. Only 0.11\% of summaries exceed 150 tokens. We limit the summaries to be less or equal to 256 tokens by limiting the maximum token generation to 256 tokens during model inference. In terms of figure structure, most figures contain between one and three subfigures, though some include up to 20.

\subsection{Textual Enrichment}
\elham{TODO: Saidul}
To enhance the dataset with more precise contextual information related to each of the subfigure images, we employed two key methods: \textit{(a)} we extracted subcaptions from the full captions corresponding to each subfigure to ensure more accurate image-text combination, and \textit{(b)} we identified in-text reference paragraphs from original articles and summarized them to further enrich the semantic content related to each of the subfigure images.
\paragraph{Subcaption Extraction}
The majority of captions in the dataset consist of multiple subcaptions, generally distinguished by delimiters such as \textit{(a)}, \textit{(b)}, or \textit{(A–F)}. Given that the total number of subfigures exceeds approximately 18 million, manual extraction of all subcaptions would not be reasonable. To address this, we adopted an automated extraction approach using a state-of-the-art open-source VLM, Qwen2.5-VL-32B-Instruct \citep{Qwen2.5-VL}. For each sample, we designed a prompt $P$ comprising the full caption $f$, a subfigure image $s$, and additional  instructions $I$ \saidul{TODO: adding reference to the prompt in appendix}. To ensure determinism and prevent hallucinations or factual inaccuracies, the model was explicitly instructed to extract a verbatim copy of the subcaption directly from the full caption, without adding any additional text or explanation. In cases where a subcaption could not be identified, the model was instructed to extract the verbatim copy of the full caption instead. To evaluate the quality of the automated extraction method, we utilized LLM-as-a-judge method using Qwen2.5-VL-32B-Instruct and assessed a representative subset of 1,000 samples. We observed approximately 6\% error, primarily due to missing subcaptions, indicating that the model performs reliably for large-scale automated subcaption extraction.

\paragraph{In-text Reference Extraction and Summarization}
Since the compound figures of \datasetsub were collected from the \biomedica dataset \citep{lozano2025biomedica}, we used the dataset’s accompanying image metadata, such as \textit{image\_context} which are textual references associated with each compound figure. However, these in-text references frequently extend across multiple paragraphs, often exceeding the model’s context length. In many cases, important contextual details appear outside the sentences that directly correspond to a subfigure, making it difficult to determine which texts are related to which subfigure. To mitigate these issues, we employed the Qwen2.5-14B-Instruct \citep{Qwen2.5-VL} model to generate concise, context-aware summaries that distill the most relevant information while retaining essential details for each subfigure. For each sample, we designed a prompt $P$ comprising the full caption $f$, a subcaption related to a subfigure image $s$, the image context $c$ and additional  instructions $I$. 





==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:Experiment}

\subsection {Encoder Pretraining}
As a first step, we train separate encoders for image and text modalities by aligning their representations using a vanilla contrastive loss. Let $\ienc$ denote an image encoder and $\tenc$ denote a text encoder that maps images and text to a common representation space, respectively. Given a batch of training samples $B = \{ (x_i, t_i)\}_{i=1}^N$, where $x_i$ and $t_i$ denote the $i^{\text{th}}$ image and text instances respectively, the InfoNCE loss \citep{oord2018representation} is optimized by minimizing the distance between the representations of an image and its corresponding text, $(\ienc(x_i), \tenc(t_i))$, while maximizing the distance between unrelated image-text representation pairs, $(\ienc(x_i), \tenc(t_j)), \hspace{1mm} i \neq j$:
\beqa
\label{eq:contrastive_loss}
\ell_{\text{con}}(x_i,t_i;B) = - \left( \log \frac{\exp(\inl \ienc(x_i), \tenc(t_i) \inr / \tau)}{\sum_{k=1}^N \exp (\inl \ienc(x_i), \tenc(\boldsymbol{t_k}) \inr / \tau)} +
 \log \frac{\exp(\inl \ienc(x_i), \tenc(t_i) \inr / \tau)}{\sum_{k=1}^N \exp (\inl \ienc(\boldsymbol{x_k}), \tenc(t_i) \inr / \tau)} \right),
\eeqa
where $\inl \cdot, \cdot \inr$ denotes similarity between two vectors (e.g. cosine similarity), and $\tau > 0$ is a temperature parameter. For simplicity of notation, we drop $B$ and denote the loss for $(x,t)$ by $\loss_\text{con}(x,t)$. Multimodal contrastive learning trains encoders $\ienc$ and $\tenc$ by minimizing Eq.~\ref{eq:contrastive_loss} over the pairs in $B$:
\beqa
\label{eq:multimodal_loss}
\loss_{\text{multimodal}} = \min_{\ienc, \tenc} \hspace{2mm} \mathbb{E}_B \Big[ \frac{1}{N} \sum_{i=1}^N  \ell_\text{con}(x_i,t_i)\Big].
\eeqa

\subsection{Evaluation Setup}\label{eval}
To systematically assess the impact of dataset scale and curation quality, we perform evaluations along both dimensions. Our models are trained under a unified architecture and training protocol to ensure controlled evaluation. For models without accessible training data, we instead use publicly released checkpoints obtained from HuggingFace. For the text encoder, we use PubMedBERT \citep{pubmedbert}, and for the vision encoder, we adopt a ViT-B/16 transformer \citep{dosovitskiy2020image} pretrained on ImageNet. The encoders are trained for 64 epochs with batch size of 2048. The best-performing checkpoints for each encoder are selected based on validation retrieval performance. The training was performed using 8 NVIDIA A100 GPUs and completed in five days. We conducted our experiments using the mmlearn
multimodal learning framework, available
at https://github.com/VectorInstitute/mmlearn/tree/main.

For assessing the role of quality, particularly subfigure-level extraction, we train a baseline model on the 6 million compound figure-caption pairs of \datasetcomp, where each compound image is used in its original form without panel separation (section \ref{detr}). We also include publicly available checkpoints from other models trained on \biomedclip \citep{zhang2023biomedclip} and \biomedica \citep{lozano2025biomedica}. For \biomedica, we use the checkpoint referred to as \texttt{BMC-CLIP}$_\text{CF}$ in \citet{lozano2025biomedica}, which is trained on a filtered subset of the full dataset. This subset retains content labeled under clinical and scientific imaging, immunoassays, illustrative diagrams, chemical structures, maps, tools and materials, and hand-drawn or screen-based visuals, while explicitly excluding tables and charts. The model is trained for 36 epochs. For \biomedclip, we use the checkpoint trained on 15 million image-caption pairs, referred to as \texttt{BioMedCLIP} in \citet{zhang2023biomedclip}. All external checkpoints were obtained from their official HuggingFace repositories and are evaluated using our standardized downstream protocols.

To further ensure consistency, we independently reproduce the PMC-OA dataset \citep{lin2023pmc} and train encoders using the same architecture and hyperparameters as those used for \datasetsub and \datasetcomp. Throughout the paper, all encoder variants are referenced by the name of the dataset on which they are trained, to facilitate transparent comparison. All the details of pretraining and hyperparameters are listed in the supplementary material.

\subsection{Downstream Tasks}
The performance of the encoders is evaluated on external and non-PMC datasets across two primary tasks: retrieval and zero-shot classification. For the retrieval task, we assess both image-to-text (I2T) and text-to-image (T2I) retrieval across three benchmark datasets representative of distinct medical imaging modalities: Quilt \citep{ikezogwo2024quilt} (microscopy), MIMIC-CXR \citep{johnson2019mimic} (radiology), and DeepEyeNet \citep{huang2021deepopht} (VLP). To evaluate robustness in retrieval, we follow established protocols from \cite{liu2024diffrect} by applying a suite of low-level visual perturbations, including brightness adjustment, spatial shift, rotation, horizontal flip, and zoom, directly to the test images. To assess the statistical significance of robustness differences, we employ the Wilcoxon signed-rank test, a non-parametric method for paired comparisons \citep{wilcoxon1945individual}. We consider a p-value less than 0.01 as statistically significant. For classification, we evaluate models using both zero-shot and linear probing protocols across a diverse set of tasks: five in radiology, eight in microscopy, and six in VLP. We use our trained vision and text encoders to encode the image and question, respectively.

\subsection{Cross-Modal Retrieval and Robustness}
Table~\ref{ret-table} summarizes the performance of various VLMs on cross-modal retrieval tasks across three benchmark datasets: MIMIC-CXR, Quilt, and DeepEyeNet. We report Recall@200 (other Recall metrics are listed in the supplementary material) for both image-to-text and text-to-image retrieval, with the final column showing the Average Recall (AR) aggregated across all tasks. Models trained on \datasetsub and even \datasetcomp (compound figures) consistently outperform \biomedclip and \biomedica, across all three tasks and retrieval directions. Among them, \datasetcomp achieves the highest AR of 21.22, while \datasetsub sets a new state-of-the-art with an AR of 21.64. This represents 31\% relative gain in average retrieval performance over \biomedclip.

Robustness, quantified as the ratio between retrieval performance under perturbations (explained in section \ref{eval}) and performance on the original data is presented in Figure~\ref{fig:ret-robust} (Right). Models trained on \datasetsub consistently achieve higher robustness scores relative to baseline models, reflecting improved performance stability under input perturbations in addition to superior retrieval performances. We observe statistically significant differences (p < 0.01) on Quilt and DeepEyeNet as shown in Figure \ref{fig:ret-robust} (Left). These findings are particularly relevant to our focus on subfigure extraction and the potential for improved robustness in imaging modalities that exhibit high visual and semantic heterogeneity.

\begin{table*}[h]
\centering
\caption{Retrieval performance (Recall@200) of all models trained on paired image-caption pairs in the medical domain. The last column, Average Recall (AR), aggregates the results across all tasks. Highest performance values are in bold, second-best are underlined. \datasetcomp refers to a baseline model trained on a filtered subset of the \biomedica dataset, using compound figures in their original form without subfigure decomposition. The \biomedica model retrieved from Hugging Face is trained on a filtered subset of the full dataset, as described in their original paper. }
{\small
\begin{tabular}{lccc|ccc|c}
\toprule
              & \multicolumn{3}{c|}{\textbf{Image-to-Text}} & \multicolumn{3}{c|}{\textbf{Text-to-Image}} & \\
\textbf{Model} & \textbf{MIMIC} & \textbf{Quilt} & \textbf{DeepEyeNet} & \textbf{MIMIC} & \textbf{Quilt} & \textbf{DeepEyeNet} & \textbf{AR} \\
\midrule
PMC-OA & 0.139 & 0.142 & 0.152 & 0.152 & 0.149 & 0.157 & 0.148 \\
\dataset & 0.17 & 0.166 & 0.183 & 0.189 & 0.162 & 0.147 & 0.17 \\
BioMedCLIP     & 0.185 & 0.165 & 0.162 & 0.162 & 0.185 & 0.146 & 0.167 \\
BIOMEDICA      & 0.076  & 0.169 & 0.155 & 0.093  & 0.195 & 0.145 & 0.139 \\
\midrule
\datasetcomp   & \textbf{0.25} & \underline{0.203} & \underline{0.172} & \textbf{0.257} & \underline{0.22} & \underline{0.170} & \underline{0.212} \\
\datasetsub    & \underline{0.226} & \textbf{0.211} & \textbf{0.196} & \underline{0.239} & \textbf{0.233} & \textbf{0.193} & \textbf{0.216} \\
\bottomrule
\end{tabular}
}
\label{ret-table}
\end{table*}

% \begin{figure}[tb]
% \centering
% \includegraphics[width=0.95\textwidth]{figure/ret-robust.pdf}
% \caption{}
% \label{fig:robustness}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figure/new-ret-robust.pdf}
%     \caption{\textbf{Left} Average robustness ratio across three retrieval benchmarks, defined as the ratio of retrieval performance under visual perturbations to that on original (unperturbed) data. \textbf{Right} Paired statistical comparisons (Wilcoxon signed-rank test) between \datasetsub and each baseline model. Results show statistically significant improvements (p < 0.01) on DeepEyeNet and Quilt for at least one baseline comparison, while differences on MIMIC-CXR are not statistically significant across any of the baselines.}
%     \label{fig:ret-robust}
% \end{figure}


\begin{figure}[h]
    \centering
    \begin{minipage}{0.45\textwidth}
        \includegraphics[width=\textwidth]{figure/robust.pdf}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.5\textwidth}
        \caption{\textbf{Up:} Average robustness ratio across three retrieval benchmarks, defined as the ratio of performance under visual perturbations to that on original (unperturbed) data. Higher values indicate greater robustness to noise and distortion. \textbf{Down:} Paired statistical comparisons (Wilcoxon signed-rank test) between \datasetsub and each baseline model. Results show statistically significant improvements ($p < 0.01$) on DeepEyeNet and Quilt for at least one baseline, while differences on MIMIC-CXR are not statistically significant, suggesting similar robustness across models in that domain. These findings highlight the importance of pretraining choices in domains with fine-grained visual features.}
        \label{fig:ret-robust}
    \end{minipage}
\end{figure}


\negin{

From my thesis:

The robustness evaluation reveals that models trained on OPEN-PMC exhibit consistently stronger resilience to visual perturbations compared to all baseline models. Across radiology (MIMIC-CXR), microscopy (Quilt), and visible light (DeepEyeNet) benchmarks, retrieval performance for OPEN-PMC-18M remains stable under transformations such as brightness adjustments, shifts, rotations, flips, and zoom distortions. When normalized against performance on unaltered images, OPEN-PMC-18M achieves the highest robustness ratios across all modalities, demonstrating that its embeddings generalize more reliably under non-ideal imaging conditions.  

Quantitatively, OPEN-PMC-18M maintains retrieval accuracy within a narrow margin of its clean-image baseline, whereas models trained on PMC-OA and BIOMEDICA show pronounced drops, particularly for microscopy and visible light tasks. For example, robustness on Quilt improves by more than 15\% relative to BioMedCLIP, while robustness on DeepEyeNet improves by over 20\%. Even the intermediate OPEN-PMC-2M model outperforms larger baselines, showing that the benefits of subfigure-level curation extend beyond accuracy to stability under perturbations.  

Statistical analysis using the Wilcoxon signed-rank test confirms that the robustness improvements of OPEN-PMC-18M over PMC-OA, BIOMEDICA, and BioMedCLIP are significant at the $p < 0.01$ level. This result establishes that the observed gains are not due to random variation, but rather reflect the effect of dataset fidelity on representation quality.  

Together, these findings demonstrate that OPEN-PMC-18M not only achieves state-of-the-art retrieval and zero-shot classification performance but also produces representations that are substantially more robust. This robustness is particularly important in biomedical applications, where variations in acquisition devices, preprocessing pipelines, and imaging conditions are inevitable. By improving stability across perturbations, OPEN-PMC-trained models provide a more reliable foundation for real-world deployment in diverse clinical and research settings.

\begin{table}[htb]
\centering
\caption{Robustness evaluation across retrieval benchmarks. Robustness is quantified as the ratio of performance under visual perturbations (brightness, shift, rotation, flip, zoom) to performance on the original test set. Higher values indicate greater stability to perturbations. Statistically significant improvements of OPEN-PMC-18M over baselines (p $<$ 0.01, Wilcoxon signed-rank test) are marked with *.}
\label{tab:robustness}
\begin{tabular}{lccc|c}
\toprule
\textbf{Model} & \textbf{MIMIC-CXR} & \textbf{Quilt} & \textbf{DeepEyeNet} & \textbf{Average Robustness} \\
\midrule
PMC-OA        & 0.86 & 0.72 & 0.68 & 0.75 \\
BioMedCLIP    & 0.88 & 0.74 & 0.70 & 0.77 \\
BIOMEDICA     & 0.84 & 0.71 & 0.67 & 0.74 \\
\midrule
PMC-6M        & 0.91 & 0.78 & 0.74 & 0.81 \\
OPEN-PMC-18M  & \textbf{0.92} & \textbf{0.85}* & \textbf{0.82}* & \textbf{0.86}* \\
\bottomrule
\end{tabular}
\end{table}
}



\subsection{Zero-shot Classification}
Model comparisons for zero-shot classification are presented in Table~\ref{zsc-tab}, and linear probing results are provided in the supplementary material. Results are grouped and averaged by modality. Models trained on \datasetsub consistently achieve the highest average performance across modalities, demonstrating superior transferability relative to all other evaluated models. Across the full set of 18 classification tasks spanning radiology, microscopy, and VLP , \datasetsub ranks first in 6 tasks and second in 2. A similar trend is observed in the linear probing results, where \datasetsub also achieves the highest average performance across modalities.









\begin{table*}[h!]
    \caption{Zero-shot classification F1-scores across diverse medical datasets for different models. For details on model training configurations and dataset sources, refer to the retrieval results table and its caption (Table~\ref{ret-table}).}
    \label{tab:ZSC_F1}
    \centering
    \begin{tabular}{lcccccc}
    \toprule
      &\multicolumn{5}{c}{\textbf{Radiology}} \\
     \textbf{Model} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PneumoniaMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont BreastMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OrganAMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OrganCMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OrganSMNIST+}}} & Average \\
    \midrule
    PMC-OA           & 50.94 & 52.36 & 19.70 & 14.79 & 16.99 & 30.95 \\
    \dataset         & 50.13 & \textbf{59.65} & \textbf{27.95} & \textbf{23.23} & \textbf{20.03} & \underline{36.19} \\
    BioMedCLIP       & 60.13 & 33.76 & 19.40 & 14.12 & 16.00 & 28.62 \\
    BIOMEDICA        & 38.46 & \textbf{56.66} & 19.25 & \underline{17.13} & 16.33 & 29.56 \\
    \midrule
    \datasetcomp     & \underline{68.81} & 26.87 & \underline{23.48} & 14.68 & \underline{17.57} & 30.28 \\
    \datasetsub      & \textbf{86.18} & \underline{50.36} & 18.75 & 14.33 & 13.65 & \textbf{36.65} \\
    \end{tabular}

    \begin{tabular}{lccccccc}
    \toprule
     &\multicolumn{6}{c}{\textbf{Visible Light 
 Photography}} \\
     \textbf{Model} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PAD-UFES-20}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont Skin Cancer}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PathMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont DermaMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont OCTMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont RetinaMNIST+}}} & Average \\
    \midrule
    PMC-OA           & 17.18 & 13.30 & \underline{56.03} & 14.29 & \textbf{50.74} & \textbf{27.22} & 29.79 \\
    \dataset           & 21.11 & 13.56 & 49.16 & 14.60 & 45.27 & \underline{26.12} & 28.30\\
    BioMedCLIP        & 24.41 & 13.62 & 42.27 & 14.07 & 11.87 & 20.82 & 21.17 \\
    BIOMEDICA       & \textbf{40.57} & \underline{17.20} & 49.10 & \textbf{21.89} & 10.00 & 18.53 & 26.21 \\
    \midrule
    \datasetcomp     & \underline{33.04} & 16.56 & 52.17 & \underline{17.52} & \underline{46.91} & 22.81 & \underline{31.50} \\
    \datasetsub     & 24.38 & \textbf{18.28} & \textbf{60.75} & 17.01 & 46.28 & 23.15 & \textbf{31.64} \\
    \end{tabular}

    \begin{tabular}{lccccccccc}
    \toprule
     &\multicolumn{8}{c}{\textbf{Microscopy}} \\
     \textbf{Model} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont Sicap}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont PCam}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont NCT-CRC-HE}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont LC-Lung}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont LC-Colon}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont BACH}}} &  {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont BloodMNIST+}}} & {\rotatebox{0}{\textbf{\fontsize{7}{7}\selectfont TissueMNIST+}}} & Average \\
    \midrule
    PMC-OA           & \underline{32.80} & \underline{70.65} & 43.95 & 56.04 & \textbf{91.05} & 33.75 & 5.57 & \textbf{7.17} & 42.62\\
    \dataset          & 20.71 & 38.96 & 42.88 & 63.97 & \underline{88.38} & 41.31 & \underline{10.73} & \underline{6.08} & 39.12 \\
    BIOMEDICA        & 31.80 & 62.17 & 48.98 & 70.93 & 84.43 & 39.83 & 4.37 & 4.31 & 43.35 \\
    BioMedCLIP       & \textbf{41.53} & \textbf{72.57} & 49.46 & 76.63 & 86.54 & 23.88 & 6.83 & 3.86 & 45.16 \\
    \midrule
    \datasetcomp     & 22.89 & 68.05 & \underline{55.28} & \textbf{86.86} & 78.41 & \underline{52.58} & 3.72 & 3.05 & \underline{46.35} \\
    \datasetsub      & 16.29 & 69.55 & \textbf{64.42} & \underline{86.01} & 71.94 & \textbf{67.94} & \textbf{28.42} & 3.74 & \textbf{51.03} \\
    \bottomrule
    \end{tabular}
    \label{zsc-tab}
\end{table*}








\subsection{Representations Analysis}
To explore differences in the structure of learned image representations, we project the embedding spaces of three benchmark sets, each constructed by combining datasets used for retrieval and zero-shot classification across radiology, microscopy, and visible light photography (VLP), into two dimensions using t-SNE (Figure~\ref{fig:tsne}). The radiology benchmark includes MIMIC-CXR and other related zero-shot classification tasks, totaling approximately 41,000 samples. The microscopy and VLP benchmarks contain approximately 20,000 and 6,000 samples, respectively. To quantify differences between the embedding distributions, we compute the Maximum Mean Discrepancy (MMD) \cite{gretton2012kernel}. Given a dataset $X$ (e.g., all radiology samples), we extract embeddings $\phi(X)$ and $\psi(X)$ using vision encoders $\phi$ and $\psi$ trained on \datasetsub and \datasetcomp, respectively. To assess whether the differences between these distributions are statistically significant, we perform a permutation test by randomly reassigning samples and recomputing MMD over 100 iterations to generate an empirical null distribution.

Visual inspection of the embeddings reveals distinct representational structures between the two models. This distinction is particularly evident in microscopy and VLP, where the latent spaces of the two models are more clearly differentiated. In contrast, radiology embeddings appear more intermixed, with less visual separation between the models’ representation spaces. Nonetheless, the MMD analysis confirms that the observed differences are statistically significant across all modalities. For the aggregated radiology dataset, the observed MMD is 0.0214 (null range: 0.0186–0.0214; \textit{p} = 0.005). For the aggregated microscopy dataset, the observed MMD is 0.0212 (null range: 0.0188–0.0212; \textit{p} < 0.001). For the VLP dataset, the observed MMD is again 0.0214 (null range: 0.0186–0.0214; \textit{p} = 0.007). These results indicate that models trained on subfigure-level data yield significantly different representation spaces compared to those trained on compound figures.

\begin{figure*}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figure/new-tsne.pdf}
    \caption{t-SNE visualizations of models embeddings trained on \datasetsub and \datasetcomp on three imaging modalities, illustrating the structure and separation of the learned representation spaces. MMD analysis reveals statistically significant differences in embedding distributions across all imaging modalities. }
    \label{fig:tsne}
\end{figure*}


\negin{


==> sec/5_ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}

In this part we want to show that how important it is to decompose the images. We show that if we just discard the compound images and only train with single images performance drops noticeably which shows the importance of decomposing the images.


I am not sure the argument that data reduction by 63\% would necessarily impact the training is valid. Since we are already talking about vast datasets, a reduction of a dataset by impurities (or noise) does not necessarily impact model training, and might, to the contrary, even improve it. I think this needs to be shown and not just argumented. I see that this might be too much to ask given the short timeline of the paper, but I think you should at least discuss this option and the implications properly.
In light of your comment, we conducted an additional experiment to address your concern regarding the impact of excluding compound images from our dataset. The results are shown in the following tables. As you can see, training only on single-panel images leads to a 50\% drop in retrieval performance across all datasets. Additionally, the model's average zero-shot classification performance across all modalities also decreases.




% Requires: \usepackage{booktabs,graphicx}
% Optional macros if you use them:
% \newcommand{\dataset}{Dataset}
% \newcommand{\datasetcomp}{Dataset-Comp}
% \newcommand{\datasetsub}{Dataset-Sub}

% Requires: \usepackage{booktabs,graphicx}
\begin{table}[h!]
  \caption{Retrieval}
  \label{tab:retrieval}
  \centering
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.1}
  \small
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lccccccc}
    \toprule
    \textbf{Model} &
    \textbf{MIMIC $(I\to T)$} &
    \textbf{Quilt $(I\to T)$} &
    \textbf{DeepEye $(I\to T)$} &
    \textbf{MIMIC $(T\to I)$} &
    \textbf{Quilt $(T\to I)$} &
    \textbf{DeepEye $(T\to I)$} &
    \textbf{Avg.\ Recall} \\
    \midrule
    Only single-panel & 0.048 & 0.158 & 0.127 & 0.045 & 0.165 & 0.111 & 0.109 \\
    Open-PMC-18M      & \textbf{0.226} & \textbf{0.211} & \textbf{0.196} & \textbf{0.239} & \textbf{0.233} & \textbf{0.193} & \textbf{0.216} \\
    \bottomrule
  \end{tabular}%
  }
\end{table}







==> sec/6_limitation.tex <==
\section{Limitations and Open Challenges in 
\label{sec:limit}

Biomedical Vision–Language Representation Learning}
Our findings suggest that in the context of VLM representation learning, data quality and dataset scale should be viewed as complementary axes in building effective and robust biomedical VLMs. Subfigure extraction, used here as a means to improve alignment quality demonstrates clear benefits, particularly in visually heterogeneous domains such as microscopy and visible light photography, as shown in Figure~\ref{fig:example}. Radiology, however, exhibits more limited gains. These observations raise the importance of modality-aware pretraining strategies, where both model architectures and data curation pipelines are adapted to the unique characteristics of each imaging modality. While our results highlight promising trends, we note that additional analysis is required, particularly in radiology, across a broader and more diverse set of downstream tasks. Such evaluation will help clarify when and where subfigure extraction yields the greatest benefit. Given the strong performance and robustness of encoders trained on \datasetsub, future work includes exploring their integration with large language model decoders for downstream tasks that require generative reasoning over visual inputs, such as medical report generation and visual question answering.

We recognize that scaling and curating large biomedical datasets brings challenges that extend beyond improving model performance. To support transparency and reproducibility, we release all dataset filtering criteria, subfigure detection models, and training pipelines. However, interpretability remains an open challenge in VLMs and particularly in the biomedical domain. Although our models are not intended for clinical deployment, they could be fine-tuned or adapted for various clinical application. However, without rigorous validation and careful consideration of clinical safety, such use poses serious risks. Furthermore, our datasets, sourced from open-access repositories such as PMC, may reflect underlying biases tied to specific institutions, imaging protocols, or publication norms. These factors can influence model behavior in subtle ways, limiting generalizability, especially when applied to underrepresented populations or distinct clinical settings. 



==> sec/7_conclusion.tex <==
\section{Conclusion}
In this paper we addressed a critical gap in the design of high-fidelity multimodal medical datasets, aiming to advance robust and generalizable representation learning. We evaluated the effectiveness and robustness of subfigure extraction. We introduced \datasetsub, one of the largest and highest quality image-caption pairs to date. Models trained on \datasetsub consistently outperform existing benchmarks across radiology, microscopy, and visible light photography. These findings lay the groundwork for more generalizable medical VLMs and better aligned with the complex realities of biomedical data.
